On Measuring the Intrinsic Few-Shot Hardness of Datasets

While advances in pre-training have led to dramatic improvements in few-shot learning of NLP tasks, there is limited understanding of what drives successful few-shot adaptation in datasets. In particular, given a new dataset and a pre-trained model, what properties of the dataset make it \emph{few-shot learnable} and are these properties independent of the specific adaptation techniques used? We consider an extensive set of recent few-shot learning methods, and show that their performance across a large number of datasets is highly correlated, showing that few-shot hardness may be intrinsic to datasets, for a given pre-trained model. To estimate intrinsic few-shot hardness, we then propose a simple and lightweight metric called "Spread" that captures the intuition that few-shot learning is made possible by exploiting feature-space invariances between training and test samples. Our metric better accounts for few-shot hardness compared to existing notions of hardness, and is ~8-100x faster to compute.

==> EMNLP 2022/macros.tex <==
\newcommand{\Red}[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand{\Blue}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
\newcommand{\Green}[1]{\textcolor[rgb]{0.00,0.80,0.00}{#1}}
\newcommand{\Black}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\newcommand{\Gold}[1]{\textcolor[rgb]{0.72,0.53,0.04}{#1}}

\newcommand{\chris}[1]{\Red{#1}}
\newcommand{\xr}[1]{\Green{#1}}
\newcommand{\smurty}[1]{\Blue{#1}}

\newcommand{\lmtt}[1]{\fontfamily{lmtt}\selectfont{#1}}
\newcommand{\lmss}[1]{\fontfamily{lmss}\selectfont{#1}}

\newcommand{\dat}[1]{\lmss{#1}}


\newcommand{\fsglue}{\dat{FS-GLUE}}
\newcommand{\fsnli}{\dat{FS-NLI}}


\newcommand{\msa}{\metricn_{\text{sensitivity}}}
\newcommand{\mrda}{\metricn_{\text{RDA}}}
\newcommand{\mspread}{\metricn_{\text{\spread{}}}}



\newcommand{\spread}{\lmtt{Spread}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\dataset}[1]{\mathcal{D}_{#1}}
\newcommand{\metricn}{h}
\newcommand{\metric}[1]{\h(#1)}
\newcommand{\smetric}[2]{h_{#2}(#1)}


\newcommand{\model}{f}
\newcommand{\modeln}[1]{f(#1)}
\newcommand{\train}{\mathcal{D}_{tr}}
\newcommand{\test}{\mathcal{D}_{ts}}

\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\egg}{e.g.,}
\newcommand{\iee}{i.e.,}
\newcommand{\mfh}{\ensuremath{\mathrm{MFH}}}
\newcommand{\ifh}{\ensuremath{\mathrm{IFH}}}



% Chris's comments. At the end you can turn this off either by changing the below line to \commentsfalse or deleting all \cm.* commands and this block.
\newif\ifcomments
\commentstrue
\ifcomments
\usepackage[normalem]{ulem}
\definecolor{CMpurple}{rgb}{0.6,0.18,0.64}
\newcommand\cm[1]{\textcolor{CMpurple}{\textsf{\scriptsize[\textbf{CM\@:} #1]}}}
\newcommand\cmi[1]{\textcolor{CMpurple}{#1}}
\newcommand\cmm[1]{\marginpar{\raggedright\tiny\textcolor{CMpurple}{\textsf{{\bfseries CM\@:} #1}}}}
\newcommand\cms{\bgroup\markoverwith{\textcolor{CMpurple}{\rule[.4ex]{2pt}{0.8pt}}}\ULon}
\else
\newcommand\cm[1]{}
\newcommand\cmi[1]{\ignorespaces}
\newcommand\cmm[1]{}
\newcommand\cms[1]{#1}
\fi



